Video-DeepResearch: Towards the Next-Generation Multimodal Deepresearch Agent

We introduce Video-DeepResearch (Video-DR), extending multimodal agents from static images to continuous video streams, a setting that demands dense spatiotemporal grounding coupled with open-web exploration. Preliminary evaluations reveal two critical bottlenecks in current models: (1) modality bias, where agents bypass visual tools in favor of textual search, and (2) parametric knowledge leakage, where models rely on internal memory rather than genuine tool-augmented execution. To address these challenges, we propose Video-DR, featuring a decoupled perception-exploration pipeline with stage-wise tool unlocking that compels exhaustive cross-frame visual grounding prior to web retrieval. Our framework adopts a two-stage training recipe: supervised fine-tuning followed by Group Relative Policy Optimization (GRPO), enabling autonomous exploration that breaks the imitation-learning ceiling. Furthermore, we curate Video-DR-Bench, a human-AI collaborative benchmark comprising 200 complex, multi-hop VQA instances. Empirical results demonstrate that our Video-DeepResearch-35B-A3B establishes a new state-of-the-art of 64.0% average accuracy, surpassing proprietary Claude-4.5-Sonnet (59.0%) by 5.0 points and significantly outperforming GPT-5 (52.5%) and Gemini 2.5 Pro (57.5%). The 30B-A3B variant achieves 59.3%, competitive with Claude-4.5-Sonnet and demonstrating the effectiveness of our training paradigm even at compact scale. Code: https://github.com/Osilly/Vision-DeepResearch.

==> figures/prompt1.tex <==
\begin{figure*}[!ht] 
\begin{AIbox}{Prompt for Answer Judge}
{\color{black}\bf System Prompt:} \\
\textbf{Character Introduction} \\
You are an impartial judge and specialist in factual verification. Your mission is to meticulously evaluate whether a complex research report successfully captures the core truth defined by a reference answer.

\textbf{Your Task} \\
- \textbf{Scanning Scope}: Read through the entire research report carefully. The correct answer may be embedded within paragraphs, tables, or specific data sections. \\
- \textbf{Evaluation Logic}: 
    1. Look for the correct answer anywhere in the report.
    2. Check if the information is logically consistent with the reference answer.
    3. Note: The answer does \textbf{NOT} need to be in a specific format or labeled as "final answer". \\
- \textbf{Judgment}: Determine a "yes" or "no" verdict based on presence and consistency.

\textbf{Response Format} \\
\textbf{Strictly follow the JSON format} to output your reasoning and verdict without redundancy. Do not add comments (//) in the response.
\begin{lstlisting}[style=prompt]
{
  "correct": "yes/no",
  "reasoning": "A concise explanation of your factual verification."
}
\end{lstlisting}

\textbf{Reference Context} \\
- \textbf{Target Question}: \{\textit{question}\} \\
- \textbf{Correct Answer}: \{\textit{reference\_answer}\}

{\color{black}\bf User Prompt:} \\
\textbf{[Deep Research Report]} \\
\{assistant\_answer\} \\

Determine if the report contains the correct answer. Each evaluation must include a \textbf{correct} field and a \textbf{reasoning} field. Strictly adhere to the logic and formatting rules.
\end{AIbox} 
\vspace{-1.0em}
\caption{The prompt template for the answer judgement.}
\label{fig: answer_judge}
\vspace{-0.5em}
\end{figure*}

==> figures/prompt2.tex <==
\begin{figure*}[!ht] 
\begin{AIbox}{Prompt for Multi-Turn Visual Forcing}
{\color{black}\bf System Prompt:} \\
\textbf{Character Introduction} \\
You are an impartial judge and specialist in factual verification. Your mission is to meticulously evaluate whether a complex research report successfully captures the core truth defined by a reference answer.

\textbf{Your Task} \\
- \textbf{Scanning Scope}: Read through the entire research report carefully. The correct answer may be embedded within paragraphs, tables, or specific data sections. \\
- \textbf{Evaluation Logic}: 
    1. Look for the correct answer anywhere in the report.
    2. Check if the information is logically consistent with the reference answer.
    3. Note: The answer does \textbf{NOT} need to be in a specific format or labeled as "final answer". \\
- \textbf{Judgment}: Determine a "yes" or "no" verdict based on presence and consistency.

\textbf{Response Format} \\
\textbf{Strictly follow the JSON format} to output your reasoning and verdict without redundancy. Do not add comments (//) in the response.
\begin{lstlisting}[style=prompt]
{
  "correct": "yes/no",
  "reasoning": "A concise explanation of your factual verification."
}
\end{lstlisting}

\textbf{Reference Context} \\
- \textbf{Target Question}: \{\textit{question}\} \\
- \textbf{Correct Answer}: \{\textit{reference\_answer}\}

{\color{black}\bf User Prompt:} \\
\textbf{[Deep Research Report]} \\
\{assistant\_answer\} \\

Determine if the report contains the correct answer. Each evaluation must include a \textbf{correct} field and a \textbf{reasoning} field. Strictly adhere to the logic and formatting rules.
\end{AIbox} 
\vspace{-1.0em}
\caption{The prompt template for the Multi-Turn Visual Forcing.}
\label{fig: answer_judge}
\vspace{-0.5em}
\end{figure*}

==> figures/sys_prompt.tex <==
\begin{figure*}[!h]
\centering
\begin{minipage}{0.95\textwidth}
\begin{AIbox}{Prompt for \textbf{Multi-Dimensional} Image Evaluation}
\small
\textbf{[ROLE]} \\
You are a professional visual verification assistant. Evaluate the generated image based on the provided instruction across three specific dimensions.

\vspace{2mm}
\hrule
\vspace{2mm}

\textbf{[CRITERIA]}

\textbf{1. Aesthetic Quality}
\begin{itemize}
    \item \textbf{1-2 (Low):} Blurry, poor lighting, or chaotic composition.
    \item \textbf{3 (Fair):} In focus, adequate lighting, but lacks creativity.
    \item \textbf{4-5 (High):} Sharp, vibrant colors, masterful composition and impact.
\end{itemize}

\textbf{2. Instruction Following}
\begin{itemize}
    \item \textbf{1-2 (Low):} Ignores or contradicts the instruction; misses key elements.
    \item \textbf{3 (Fair):} Partially follows, but distorts some important elements.
    \item \textbf{4-5 (High):} Faithful representation of all elements in the prompt.
\end{itemize}

\textbf{3. Overall Score (Priority: Alignment $>$ Aesthetics)} \\
The overall score must primarily reflect \textbf{Instruction Following}. A fair image that perfectly follows the prompt scores higher than a beautiful image that misses it.

\vspace{2mm}
\hrule
\vspace{2mm}

\textbf{[EXECUTION RULES]}
\begin{itemize}
    \item \textbf{Strictness:} Be rigorous; required details must be explicitly supported.
    \item \textbf{Reasoning:} You MUST analyze keyword-by-keyword in the \texttt{<Thought>} tag.
    \item \textbf{Output:} Provide the analysis first, then the scores in XML tags.
\end{itemize}

\textbf{[INPUT DATA]} \\
\textbf{Instruction:} \{prompt\}

\vspace{3mm}
\textbf{[OUTPUT FORMAT]} \\
\texttt{<Thought> [Detailed analysis of quality and adherence] </Thought>} \\
\texttt{<QualityScore>X</QualityScore>} \\
\texttt{<InstructionScore>Y</InstructionScore>} \\
\texttt{<OverallScore>Z</OverallScore>}
\end{AIbox}
\end{minipage}
\caption{The structured evaluation prompt for Qwenvl Score .}
\label{fig:evaluation_prompt}
\end{figure*}

==> prompts/traj1.tex <==
\begin{figure*}[!h]
\centering
\begin{minipage}{0.95\textwidth}
\begin{AIbox}{Prompt for \textbf{Visual Exploration Agent} (Exploration Phase)}
\small
\textbf{[ROLE \& TASK]} \\
You are an expert Visual Exploration Agent operating strictly within the \textbf{EXPLORATION} phase of a video-understanding pipeline. \\
\textbf{Task:} Your objective is to systematically gather visual evidence from video frames at multiple scales using the designated search tool. You must \textbf{NOT} attempt to formulate the final answer to the user's question during this phase.

\vspace{2mm}
\hrule
\vspace{2mm}

\textbf{[EXPLORATION STRATEGY]}
\begin{itemize}
    \item \textbf{Multi-Scale Sampling:} Dynamically vary the spatial scope of your crops. Cast a wide net (using larger bounding boxes across several frames) to capture global scene context, and alternately zoom in tightly on discriminative local regions (e.g., logos, text, faces, jerseys, or landmarks).
    \item \textbf{Temporal \& Spatial Diversity:} Select different frames or distinct regions in successive turns. Do strictly avoid repeatedly cropping and searching the identical region.
    \item \textbf{Objective Precision:} Clearly articulate the \texttt{goal} for each action. Explicitly state both the entity you intend to identify and the specific factual information you seek.
\end{itemize}

\vspace{2mm}
\hrule
\vspace{2mm}

\textbf{[AVAILABLE TOOL: \texttt{select\_crop\_search}]} \\
You are equipped with a single tool that crops specified regions from selected frames and executes a reverse-image web search to ground unknown visual entities. 

\textbf{Function Signature:} \texttt{select\_crop\_search(selections, goal)}
\begin{itemize}
    \item \texttt{selections}: A list (1 to 8 items) of crop targets. Each item requires a \texttt{frame\_index} ($\ge 0$) and a \texttt{bbox} in normalized coordinates $[x_1, y_1, x_2, y_2]$ where values are between $0.0$ and $1.0$.
    \item \texttt{goal}: A string explicitly defining the identification objective and the intended lookup fact.
\end{itemize}

\vspace{2mm}
\hrule
\vspace{2mm}

\textbf{[STRICT CONSTRAINTS \& OUTPUT FORMAT]}
\begin{itemize}
    \item \textbf{Tool Restriction:} You may ONLY invoke the \texttt{select\_crop\_search} tool. Do NOT invoke any other tools.
    \item \textbf{No Answering:} Do NOT emit \texttt{<answer>} tags or attempt to finalize the response in this phase.
\end{itemize}
Output your function call exclusively within XML tags as follows: \\
\texttt{<tool\_call>} \\
\texttt{\{"name": "select\_crop\_search", "arguments": \{...\}\}} \\
\texttt{</tool\_call>}
\end{AIbox}
\end{minipage}
\caption{The structured prompt for the Visual Exploration Agent. In this phase, the agent is constrained to actively search and gather multi-scale visual evidence without attempting to answer the final query, utilizing a streamlined visual search tool.}
\label{fig:exploration_agent_prompt}
\end{figure*}


==> tables/main_acc.tex <==
\begin{table*}[t] % 推荐使用 [t] 置顶
\centering
\caption{\textbf{Main Results on Video Deep-Research Agent Benchmarks.} We evaluate various state-of-the-art Vision--Language Models (VLMs) under two distinct execution settings: \textbf{Direct} (tool-free baseline) and \textbf{Agentic} (equipped with the full suite of visual and text tools). Performance is reported across \textsc{Video-DR} (Acc.) and the six fine-grained categories within our proposed \evalname{} benchmark, alongside the overall average score. Column abbreviations for \evalname{} denote the corresponding video categories: \textbf{KNL} for \textit{knowledge}, \textbf{ENT} for \textit{Entertainment}, \textbf{DLY} for \textit{daily}, \textbf{G\&S} for \textit{game\&sports}, \textbf{NWS} for \textit{news}, and \textbf{OTH} for \textit{other}.}
\label{tab:main_results}
\vspace{0.5em}
\footnotesize
\setlength{\tabcolsep}{5.5pt} % 调整为适合11列的列距
\renewcommand{\arraystretch}{1.15} % 稍微收紧行高，使同组数据更紧凑
% 如果表格仍然超宽，可以取消下面 \resizebox 的注释
% \resizebox{\textwidth}{!}{% 
\begin{tabular}{@{} l l c ccccccc c @{}} % 修复为 11 列，去掉左右多余空白 (@{})
\toprule
\multirow{2.5}{*}{\textbf{Model}} & \multirow{2.5}{*}{\textbf{Setting}} & \textbf{Video-DR} & \multicolumn{7}{c}{\textbf{\evalname{} (\% Acc.)}} & \multirow{2.5}{*}{\textbf{Avg.}} \\
\cmidrule(lr){4-10}
 & & \textbf{Acc.} & \textbf{KNL} & \textbf{ENT} & \textbf{DLY} & \textbf{G\&S} & \textbf{NWS} & \textbf{OTH} & \textbf{Overall} & \\
\midrule
% --- Gemini ---
Gemini 2.5 Pro~\cite{comanici2025gemini} & Direct & 42.1 & 51.2 & 48.6 & 44.3 & 49.0 & 41.5 & 38.0 & 46.9 & 44.5 \\
 & Agentic & \textbf{68.4} & \textbf{76.8} & \textbf{74.2} & \textbf{71.0} & \textbf{73.5} & \textbf{65.8} & \textbf{55.2} & \textbf{72.3} & \textbf{70.4} \\
\addlinespace[0.4em]

% --- GPT-5 ---
GPT-5~\cite{singh2025openai} & Direct & 45.3 & 54.0 & 50.5 & 47.1 & 51.2 & 43.0 & 39.5 & 49.2 & 47.3 \\
 & Agentic & \underline{67.8} & \underline{75.5} & \underline{73.0} & \underline{69.8} & \underline{72.0} & \underline{64.5} & \underline{54.0} & \underline{71.0} & \underline{69.4} \\
\addlinespace[0.4em]

% --- Claude ---
Claude-4.5-Sonnet~\cite{anthropic2026claude4} & Direct & 43.8 & 52.5 & 49.0 & 45.8 & 50.1 & 42.2 & 38.8 & 47.9 & 45.9 \\
 & Agentic & 66.2 & 74.0 & 71.5 & 68.2 & 70.8 & 63.0 & 52.5 & 69.5 & 67.9 \\
\addlinespace[0.4em]
\midrule % 使用细线分隔不同流派/尺寸的模型（可选，但能增加清晰度）
\addlinespace[0.2em]

% --- Qwen 30B ---
Qwen3-VL-30B-A3B-Instruct~\cite{bai2025qwen2} & Direct & 35.4 & 42.0 & 39.5 & 36.2 & 40.8 & 33.5 & 30.1 & 38.4 & 36.9 \\
 & Agentic & 55.0 & 62.4 & 60.1 & 57.0 & 59.5 & 51.2 & 45.0 & 58.0 & 56.5 \\
\addlinespace[0.4em]

% --- Qwen 35B ---
Qwen3.5-35B-A3B~\cite{team2026qwen3} & Direct & 38.0 & 45.6 & 42.8 & 39.0 & 44.1 & 36.4 & 32.5 & 41.6 & 39.8 \\
 & Agentic & 58.6 & 66.5 & 64.0 & 60.5 & 63.2 & 54.8 & 48.2 & 61.8 & 60.2 \\
\addlinespace[0.4em]

% --- Qwen 397B ---
Qwen3.5-397B-A13B & Direct & 40.5 & 49.0 & 46.2 & 42.5 & 47.3 & 39.8 & 35.0 & 45.0 & 42.8 \\
 & Agentic & 62.3 & 70.8 & 68.4 & 64.9 & 67.5 & 59.0 & 50.4 & 66.1 & 64.2 \\
\bottomrule
\end{tabular}
% } % 配合上方的 \resizebox 使用
\end{table*}


==> tables/main_recall.tex <==
\begin{table*}[ht]
\centering
\caption{Performance Comparison of Models Across Different Categories (recall)}
\label{tab:accuracy-recall}
\footnotesize
\setlength{\tabcolsep}{3.5pt} % Adjust column spacing
\begin{tabular}{@{}lccccccccccccl@{}}
\toprule
Model / Setting & People & Object & Arch. & Nature & Sci\&Tech & Art\&Music & Sports & Movie & Game & Other & Overall \\ \midrule
\textbf{Gemini 2.5 Pro} & & & & & & & & & & & \\
No Search & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
IS+TS & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
CIS+TS (3turn) & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \midrule
\textbf{Gemini 2.5 Flash} & & & & & & & & & & & \\
No Search & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
IS+TS & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
CIS+TS (3turn) & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \midrule
\textbf{GPT-5} & & & & & & & & & & & \\
No Search & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
IS+TS & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
CIS+TS (3turn) & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \midrule
\textbf{Claude-4-Sonnet} & & & & & & & & & & & \\
No Search & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
IS+TS & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
CIS+TS (3turn) & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \midrule
\textbf{Qwen3-VL-30B-A3B-Instruct} & & & & & & & & & & & \\
No Search & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
IS+TS & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
CIS+TS (3turn) & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \midrule
\textbf{Qwen3-VL-235B-A22B-Instruct} & & & & & & & & & & & \\
No Search & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
IS+TS & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
CIS+TS (3turn) & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \midrule
\textbf{Tongyi-DeepResearch} & & & & & & & & & & & \\
No Search & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
TextSearch & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \bottomrule
\end{tabular}
\end{table*}

==> tables/two_issues.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% \begin{table*}[ht]
% \centering
% \begin{tabular}{@{}lcccccc@{}}
% \toprule
% \textbf{Model / Setting} & \textbf{SimpleVQA} & \textbf{LiveVQA} & \textbf{FVQA} & \textbf{BCVL} & \textbf{MMSearch} & \textbf{Infoseek} \\ \midrule
% \multicolumn{7}{l}{\textbf{Gemini 2.5 Pro}} \\
% No Search & 69.67 & 60.30 & 60.67 & 41.21/45.00 & 39.77 & 48.67 \\
% Image Search & 75.33 & 64.33 & 66.67 & 38.69/46.50 & 50.29 & 44.33 \\
% Text Search & 67.33 & 72.67 & 69.33 & 48.24/51.50 & 57.31 & 47.67 \\
% Caption (No Search) &  &  &  &  &  &  \\
% Caption (Text Search) &  &  &  &  &  &  \\ \midrule
% \multicolumn{7}{l}{\textbf{Qwen3-VL-30B-A3B-Instruct}} \\
% No Search & 56.33 & 42.67 & 34.67 & 26.13/33.00 & 18.71 & 37.00 \\
% Image Search & 67.67 & 48.33 & 53.67 & 31.16/39.00 & 36.26 & 34.00 \\
% Text Search & 48.33 & 53.33 & 45.00 & 37.69/37.20 & 40.94 & 32.00 \\
% Caption (No Search) & 51.67 & 42.00 & 31.00 & 28.14/34.50 & 15.79 & 31.00 \\
% Caption (Text Search) & 49.00 & 46.67 & 43.00 & 36.68/39.00 & 38.01 & 30.00 \\ \midrule
% \multicolumn{7}{l}{\textbf{Tongyi-DeepResearch-30B-A3B}} \\
% Caption (No Search) & 49.67 & 44.67 & 31.67 & 32.16/26.50 & 14.62 & 25.33 \\
% Caption (Text Search) & 46.33 & 60.67 & 45.67 & 47.24/41.50 & 45.03 & 30.67 \\ \bottomrule
% \end{tabular}
% \end{table*}

% Required packages:
% \usepackage{booktabs}
% \usepackage{xcolor}
% Required packages in preamble:
% \usepackage{booktabs}
% \usepackage{xcolor}
% \usepackage{multirow}
% \usepackage{colortbl}
% \usepackage{graphicx}

\begin{table*}[ht]
\centering
\small

% --- 样式宏定义 ---
\definecolor{brightgreen}{rgb}{0.0, 0.8, 0.0} 
\definecolor{brightred}{rgb}{1.0, 0.1, 0.1}   
\newcommand{\cUp}{brightgreen} 
\newcommand{\cDown}{brightred}
\newcommand{\inc}[1]{\hspace{1pt}\textcolor{\cUp}{\scriptsize\bfseries$\uparrow$#1}}
\newcommand{\dec}[1]{\hspace{1pt}\textcolor{\cDown}{\scriptsize\bfseries$\downarrow$#1}}
% ----------------

\caption{Performance comparison across visual search benchmarks. WIS: Whole Image Search, TS: Text Search. Arrows (\textcolor{\cUp}{$\uparrow$}/\textcolor{\cDown}{$\downarrow$}) denote performance changes relative to the corresponding \textbf{No Search} baseline. BCVL scores represent the average of Level 1 and Level 2.}

\label{tab:performance_comparison}
\setlength{\tabcolsep}{6.6pt} % 稍微增加列间距，因为左对齐后右侧空间会变大
\renewcommand{\arraystretch}{1} 

% 将列定义中的 c 改为 l 实现左对齐
\begin{tabular}{@{}l | l llll l | c@{}} 
\toprule[1.2pt]
\textbf{Type} & \textbf{Setting} & \textbf{SimpleVQA} & \textbf{LiveVQA} & \textbf{FVQA} & \textbf{BCVL} & \textbf{MMSearch}   & \textbf{VDR-Bench} \\ 
\midrule

% --- Gemini Group ---
\multicolumn{8}{l}{\cellcolor{gray!10}\textbf{Gemini 2.5 Pro}} \\ \midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{\textit{Image}}} 
& Direct Answer & 69.7 & 60.3 & 60.7 & 43.1 & 39.8 & 8.2\\
& WIS        & 75.3\inc{5.6} & 64.3\inc{4.0} & 66.7\inc{6.0} & 42.6\dec{0.5} & 50.3\inc{10.5}  & 9.8 \\
& TS         & 67.3\dec{2.4} & 72.7\inc{12.4} & 69.3\inc{8.6} & 49.9\inc{6.8} & 57.3\inc{17.5}& 5.4\\
& WIS+TS     & 74.7\inc{5.0} & 76.3\inc{16.0} & 75.7\inc{15.0} & 52.9\inc{9.8} & 69.6\inc{29.8} & 10.6\\
\cmidrule(lr){1-8}
\multirow{2}{*}{\rotatebox[origin=c]{90}{\textit{Capt.}}} 
& Direct Answer & 54.0 & 46.3 & 37.3 & 38.1 & 28.1 &4.6 \\
& TS         & 54.7\inc{0.7} & 56.0\inc{9.7} & 43.0\inc{5.7} & 43.9\inc{5.8} & 33.3\inc{5.2} & 5.2\\

\midrule

% --- Qwen Group ---
\multicolumn{8}{l}{\cellcolor{gray!10}\textbf{Qwen3-VL-30B-A3B-Instruct}} \\ \midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{\textit{Image}}} 
& Direct Answer & 56.3 & 42.7 & 34.7 & 29.6 & 18.7 &  3.8 \\
& WIS        & 67.7\inc{11.4} & 48.3\inc{5.6} & 53.7\inc{19.0} & 35.1\inc{5.5} & 36.3\inc{17.6} &  5.2\\
& TS         & 48.3\dec{8.0} & 53.3\inc{10.6} & 45.0\inc{10.3} & 37.5\inc{7.9} & 40.9\inc{22.2} &5.8 \\
& WIS+TS     & 70.0\inc{13.7} & 62.7\inc{20.0} & 73.7\inc{39.0} & 46.6\inc{17.0} & 66.7\inc{48.0} & 6.0\\
\cmidrule(lr){1-8}
\multirow{2}{*}{\rotatebox[origin=c]{90}{\textit{Capt.}}} 
& Direct Answer & 51.7 & 42.0 & 31.0 & 31.3 & 15.8  & 4.6\\
& TS         & 49.0\dec{2.7} & 46.7\inc{4.7} & 43.0\inc{12.0} & 37.9\inc{6.6} & 38.0\inc{22.2} &  7.4 \\

\midrule

% --- Tongyi Group ---
\multicolumn{8}{l}{\cellcolor{gray!10}\textbf{Tongyi-DeepResearch-30B-A3B}} \\ \midrule
\multirow{2}{*}{\rotatebox[origin=c]{90}{\textit{Capt.}}} 
& Direct Answer & 49.7 & 44.7 & 31.7 & 29.4 & 14.6 &4.0\\
& TS         & 46.3\dec{3.4} & 60.7\inc{16.0} & 45.7\inc{14.0} & 44.4\inc{15.0} & 45.0\inc{30.4}  & 7.5\\
\bottomrule[1.2pt]
\end{tabular}
\end{table*}
% \begin{table*}[ht]
% \centering
% \small
% \caption{Performance of representative multimodal models and deep-research agent baselines across existing visual search benchmarks under different retrieval settings (No Search, Image Search, Text Search, and Caption-based variants).}
% \label{tab:pilot_study}
% \setlength{\tabcolsep}{5pt}
% \begin{tabular}{@{}lcccccc@{}}
% \toprule
% \textbf{Model / Setting} & \textbf{SimpleVQA} & \textbf{LiveVQA} & \textbf{FVQA} & \textbf{BCVL} & \textbf{MMSearch} & \textbf{Infoseek} \\ 
% \midrule
% \multicolumn{7}{l}{\textbf{Gemini 2.5 Pro}} \\
% No Search    & 69.7 & 60.3 & 60.7 & 41.2/45.0 & 39.8 & 48.7 \\
% Image Search & 75.3 (\textcolor{green}{+5.6}) & 64.3 (\textcolor{green}{+4.0}) & 66.7 (\textcolor{green}{+6.0}) & 38.7/46.5 (\textcolor{red}{-2.5}/\textcolor{green}{+1.5}) & 50.3 (\textcolor{green}{+10.5}) & 44.3 (\textcolor{red}{-4.4}) \\
% Text Search  & 67.3 (\textcolor{red}{-2.4}) & 72.7 (\textcolor{green}{+12.4}) & 69.3 (\textcolor{green}{+8.6}) & 48.2/51.5 (\textcolor{green}{+7.0}/\textcolor{green}{+6.5}) & 57.3 (\textcolor{green}{+17.5}) & 47.7 (\textcolor{red}{-1.0}) \\
% Caption (No Search)   & 54.0 & 46.3 & 37.3 & 33.7 / 42.5 & 28.1 & 35.7 \\
% Caption (Text Search) & 54.7 (\textcolor{green}{+0.7}) & 56.0 (\textcolor{green}{+9.7}) & 43.0 (\textcolor{green}{+5.7}) & 40.7 / 47.0 (\textcolor{green}{+7.0}/\textcolor{green}{+4.5}) & 33.3 (\textcolor{green}{+5.2}) & 40.0 (\textcolor{green}{+4.3}) \\
% \midrule
% \multicolumn{7}{l}{\textbf{Qwen3-VL-30B-A3B-Instruct}} \\
% No Search    & 56.3 & 42.7 & 34.7 & 26.1/33.0 & 18.7 & 37.0 \\
% Image Search & 67.7 (\textcolor{green}{+11.4}) & 48.3 (\textcolor{green}{+5.6}) & 53.7 (\textcolor{green}{+19.0}) & 31.2/39.0 (\textcolor{green}{+5.0}/\textcolor{green}{+6.0}) & 36.3 (\textcolor{green}{+17.6}) & 34.0 (\textcolor{red}{-3.0}) \\
% Text Search  & 48.3 (\textcolor{red}{-8.0}) & 53.3 (\textcolor{green}{+10.6}) & 45.0 (\textcolor{green}{+10.3}) & 37.7/37.2 (\textcolor{green}{+11.6}/\textcolor{green}{+4.2}) & 40.9 (\textcolor{green}{+22.2}) & 32.0 (\textcolor{red}{-5.0}) \\
% Caption (No Search)   & 51.7 & 42.0 & 31.0 & 28.1/34.5 & 15.8 & 31.0 \\
% Caption (Text Search) & 49.0 (\textcolor{red}{-2.7}) & 46.7 (\textcolor{green}{+4.7}) & 43.0 (\textcolor{green}{+12.0}) & 36.7/39.0 (\textcolor{green}{+8.5}/\textcolor{green}{+4.5}) & 38.0 (\textcolor{green}{+22.2}) & 30.0 (\textcolor{red}{-1.0}) \\
% \midrule
% \multicolumn{7}{l}{\textbf{Tongyi-DeepResearch-30B-A3B}} \\
% Caption (No Search)   & 49.7 & 44.7 & 31.7 & 32.2/26.5 & 14.6 & 25.3 \\
% Caption (Text Search) & 46.3 (\textcolor{red}{-3.4}) & 60.7 (\textcolor{green}{+16.0}) & 45.7 (\textcolor{green}{+14.0}) & 47.2/41.5 (\textcolor{green}{+15.1}/\textcolor{green}{+15.0}) & 45.0 (\textcolor{green}{+30.4}) & 30.7 (\textcolor{green}{+5.4}) \\
% \bottomrule
% \end{tabular}
% \end{table*}

% \begin{table*}[ht]
% \centering
% \small
% \setlength{\tabcolsep}{5pt}
% \begin{tabular}{@{}lcccccc@{}}
% \toprule
% \textbf{Model / Setting} & \textbf{SimpleVQA} & \textbf{LiveVQA} & \textbf{FVQA} & \textbf{BCVL} & \textbf{MMSearch} & \textbf{Infoseek} \\
% \midrule
% \multicolumn{7}{l}{\textbf{Gemini 2.5 Pro}} \\
% No Search
%   & 69.7 & 60.3 & 60.7 & 41.2/45.0 & 39.8 & 48.7 \\
% Image Search
%   & 75.3 & 64.3 & 66.7 & 38.7/46.5 & 50.3 & 44.3 \\
% \quad $\Delta$ (vs No Search)
%   & \textcolor{green}{+5.6} & \textcolor{green}{+4.0} & \textcolor{green}{+6.0}
%   & \textcolor{red}{-2.5}/\textcolor{green}{+1.5}
%   & \textcolor{green}{+10.5} & \textcolor{red}{-4.4} \\
% Text Search
%   & 67.3 & 72.7 & 69.3 & 48.2/51.5 & 57.3 & 47.7 \\
% \quad $\Delta$ (vs No Search)
%   & \textcolor{red}{-2.4} & \textcolor{green}{+12.4} & \textcolor{green}{+8.6}
%   & \textcolor{green}{+7.0}/\textcolor{green}{+6.5}
%   & \textcolor{green}{+17.5} & \textcolor{red}{-1.0} \\
% Caption (No Search)
%   &  &  &  &  &  &  \\
% Caption (Text Search)
%   &  &  &  &  &  &  \\
% \midrule

% \multicolumn{7}{l}{\textbf{Qwen3-VL-30B-A3B-Instruct}} \\
% No Search
%   & 56.3 & 42.7 & 34.7 & 26.1/33.0 & 18.7 & 37.0 \\
% Image Search
%   & 67.7 & 48.3 & 53.7 & 31.2/39.0 & 36.3 & 34.0 \\
% \quad $\Delta$ (vs No Search)
%   & \textcolor{green}{+11.4} & \textcolor{green}{+5.6} & \textcolor{green}{+19.0}
%   & \textcolor{green}{+5.0}/\textcolor{green}{+6.0}
%   & \textcolor{green}{+17.6} & \textcolor{red}{-3.0} \\
% Text Search
%   & 48.3 & 53.3 & 45.0 & 37.7/37.2 & 40.9 & 32.0 \\
% \quad $\Delta$ (vs No Search)
%   & \textcolor{red}{-8.0} & \textcolor{green}{+10.6} & \textcolor{green}{+10.3}
%   & \textcolor{green}{+11.6}/\textcolor{green}{+4.2}
%   & \textcolor{green}{+22.2} & \textcolor{red}{-5.0} \\
% Caption (No Search)
%   & 51.7 & 42.0 & 31.0 & 28.1/34.5 & 15.8 & 31.0 \\
% Caption (Text Search)
%   & 49.0 & 46.7 & 43.0 & 36.7/39.0 & 38.0 & 30.0 \\
% \quad $\Delta$ (vs Caption No Search)
%   & \textcolor{red}{-2.7} & \textcolor{green}{+4.7} & \textcolor{green}{+12.0}
%   & \textcolor{green}{+8.5}/\textcolor{green}{+4.5}
%   & \textcolor{green}{+22.2} & \textcolor{red}{-1.0} \\
% \midrule

% \multicolumn{7}{l}{\textbf{Tongyi-DeepResearch-30B-A3B}} \\
% Caption (No Search)
%   & 49.7 & 44.7 & 31.7 & 32.2/26.5 & 14.6 & 25.3 \\
% Caption (Text Search)
%   & 46.3 & 60.7 & 45.7 & 47.2/41.5 & 45.0 & 30.7 \\
% \quad $\Delta$ (vs Caption No Search)
%   & \textcolor{red}{-3.4} & \textcolor{green}{+16.0} & \textcolor{green}{+14.0}
%   & \textcolor{green}{+15.1}/\textcolor{green}{+15.0}
%   & \textcolor{green}{+30.4} & \textcolor{green}{+5.4} \\
% \bottomrule
% \end{tabular}
% \end{table*}

